Entry-Specific Matrix Estimation under Arbitrary Sampling Patterns through the Lens of Network Flows

Matrix completion tackles the task of predicting missing values in a low-rank matrix based on a sparse set of observed entries. It is often assumed that the observation pattern is generated uniformly at random or has a very specific structure tuned to a given algorithm. There is still a gap in our understanding when it comes to arbitrary sampling patterns. Given an arbitrary sampling pattern, we introduce a matrix completion algorithm based on network flows in the bipartite graph induced by the observation pattern. For additive matrices, the particular flow we used is the electrical flow and we establish error upper bounds customized to each entry as a function of the observation set, along with matching minimax lower bounds. Our results show that the minimax squared error for recovery of a particular entry in the matrix is proportional to the effective resistance of the corresponding edge in the graph. Furthermore, we show that our estimator is equivalent to the least squares estimator. We apply our estimator to the two-way fixed effects model and show that it enables us to accurately infer individual causal effects and the unit-specific and time-specific confounders. For rank-$1$ matrices, we use edge-disjoint paths to form an estimator that achieves minimax optimal estimation when the sampling is sufficiently dense. Our discovery introduces a new family of estimators parametrized by network flows, which provide a fine-grained and intuitive understanding of the impact of the given sampling pattern on the relative difficulty of estimation at an entry-specific level. This graph-based approach allows us to quantify the inherent complexity of matrix completion for individual entries, rather than relying solely on global measures of performance.

==> content/simulations.tex <==
\section{Simulations}

\cycomment{We have synthetic experiments for the additive model. We should also add data studies from the fixed effect regression on network data paper? Should we also do simulations for the rank-1 model? e.g. empirically benchmark against block methods (use fully dense blocks), message passing methods, spectral methods (on sparse blocks)}

\subsection{Synthetic Simulations}
We conduct synthetic experiments with a sparsified staircase treatment pattern as depicted in Figure~\ref{fig:staircase_treatment_matrix}. The treatment graph $\mathcal{G}(\Omega^1)$ as depicted in Figure~\ref{fig:staircase_treatment_graph} has a zig-zag pattern. For most entries $(i,j)$ there does not exist a length-3 path in the graph $\mathcal{G}(\Omega^1)$, and as a result DiD fails in this scenario. The data matrix Figure~\ref{fig:simulation_eff_res} shows a heatmap of the sum of the effective resistances for the graphs corresponding to the treatment and control observations.
%
We generate row and column fixed effects from a Gaussian distribution and set the variance of the observation noise as $\sigma^2 = 0.01$. For a given realization of the observations we compute the corresponding electrical flow estimates $\hat{\beta}_{it}^{\efe}$ for all pairs $(i,t)$. We repeat the experiment 1000 times and compute the entrywise mean squared error for each entry.
Figure~\ref{fig:ratio} shows a histogram of the ratio between the entrywise mean squared error of the EFE and the sum of the effective resistances on the treatment and control graphs. Figure~\ref{fig:simulation_MSE} shows a heatmap of the entrywise mean squared error, which visually matches the heatmap of the effective resistances as depicted in Figure~\ref{fig:simulation_eff_res}. These empirical results confirm our theoretical results as stated in Theorem \ref{thm:flow_est_upper_bound} that the estimation error is proportional to the sum of the effective resistance from the treatment and control graphs, where the multiplicative factor is determined by the variance of the observation noise $\sigma^2 = 0.01$. 

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.28\textwidth}
    \includegraphics[width=\textwidth]{MS/fig/simulation_figures/blkwht.png}
    \caption{~}
    \label{fig:staircase_treatment_matrix}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.13\textwidth}
    \includegraphics[width=\textwidth]{MS/fig/staircase_treatment_graph.pdf}
    \caption{~}
    \label{fig:staircase_treatment_graph}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.5\textwidth}
    \includegraphics[width=\textwidth]{MS/fig/simulation_figures/ratio.png}
    \caption{~} \label{fig:ratio}
    \end{subfigure}
    \caption{(a) The treatment pattern $X$ has a staircase structure which gets progressively sparser to the bottom right. (b) The corresponding treatment graph $\mathcal{G}(\Omega^1)$ has a zig-zag pattern. (b) Histogram of the ratio between the entrywise squared error and the sum of effective resistances. As predicted by our theory, the ratio is distributed as a normal distribution with mean equal to $\sigma^2 = 0.01$.}
\end{figure}


\begin{figure}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{MS/fig/simulation_figures/eff_res_heat_resize.pdf}
    \caption{~} \label{fig:simulation_eff_res}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{MS/fig/simulation_figures/MSE_heat_resize.pdf}
    \caption{~} \label{fig:simulation_MSE}
    \end{subfigure}
    \caption{We can visually verify that the entrywise squared estimation error is proportional to the effective resistances. (a) Heatmap of the sum of effective resistances in the graphs corresponding to treated and control observations. (b) Heatmap of the entrywise squared estimation error.}
    \label{fig:simulation}
\end{figure}


